FloodSQL-Bench: A Retrieval-Augmented Benchmark for Geospatially-Grounded Text-to-SQL

Existing Text-to-SQL benchmarks primarily focus on single-table queries or limited joins in general-purpose domains, and thus fail to reflect the complexity of domain-specific, multi-table and geospatial reasoning, To address this limitation, we introduce FLOODSQL-BENCH, a geospatially grounded benchmark for the flood management domain that integrates heterogeneous datasets through key-based, spatial, and hybrid joins. The benchmark captures realistic flood-related information needs by combining social, infrastructural, and hazard data layers. We systematically evaluate recent large language models with the same retrieval-augmented generation settings and measure their performance across difficulty tiers. By providing a unified, open benchmark grounded in real-world disaster management data, FLOODSQL-BENCH establishes a practical testbed for advancing Text-to-SQL research in high-stakes application domains.

==> tables/llm_rag_comparisons_old.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{lcccccccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Level 0}} 
 & \multicolumn{2}{c}{\textbf{Level 1}} 
 & \multicolumn{2}{c}{\textbf{Level 2}} 
 & \multicolumn{2}{c}{\textbf{Level 3}} 
 & \multicolumn{2}{c}{\textbf{Level 4}} 
 & \multicolumn{2}{c}{\textbf{Level 5}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\textbf{Model} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} \\
\midrule

\multicolumn{13}{l}{\textbf{Close-Source in Retrieval-Augmented SQL Generation Methods}} \\
\cmidrule(lr){1-13}
GPT-4o                  
& 0.914 & 0.962 & \textbf{0.891} & \textbf{0.957} & \underline{0.909} & \textbf{0.974} & 0.883 & \underline{0.951} & \textbf{0.904} & \textbf{0.968} & 0.919 & \textbf{0.976} \\
GPT-4.1                 
& 0.915 & 0.951 & 0.876 & 0.945 & 0.897 & 0.966 & 0.864 & 0.938 & 0.883 & 0.953 & 0.907 & 0.964 \\
GPT-5.1                 
& 0.917 & \underline{0.963} & 0.886 & \underline{0.953} & 0.899 & \underline{0.970} & 0.863 & 0.945 & 0.888 & 0.956 & 0.910 & 0.968 \\
Gemini-2.0-Flash-Lite   
& 0.897 & 0.934 & 0.869 & 0.945 & 0.907 & 0.962 & 0.885 & 0.948 & 0.889 & 0.954 & 0.914 & 0.964 \\
Gemini-2.5-Flash-Lite   
& 0.885 & 0.945 & 0.846 & 0.934 & 0.906 & 0.967 & 0.855 & 0.937 & 0.876 & 0.944 & 0.901 & 0.958 \\
Gemini-2.5-Pro          
& 0.887 & 0.943 & 0.872 & 0.952 & \textbf{0.914} & \textbf{0.974} & 0.862 & 0.940 & 0.881 & 0.954 & 0.923 & 0.970 \\
%Gemini-3-Pro-Preview    
%& -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Claude-3-Haiku          
& \underline{0.919} & 0.957 & 0.862 & 0.939 & 0.895 & 0.960 & 0.870 & 0.947 & 0.890 & 0.958 & 0.895 & 0.960 \\
Claude-3.5-Haiku        
& 0.903 & 0.949 & 0.851 & 0.934 & 0.899 & 0.969 & 0.833 & 0.933 & 0.895 & \underline{0.962} & 0.899 & 0.966 \\
Claude-4.5-Haiku        
& 0.900 & 0.952 & 0.870 & 0.938 & 0.896 & 0.966 & 0.879 & 0.949 & 0.893 & 0.959 & 0.921 & 0.973 \\
Claude-4.5-Sonnet         
& 0.907 & 0.950 & 0.856 & 0.931 & 0.904 & 0.969 & \underline{0.890} & \underline{0.951} & \underline{0.898} & 0.953 & \underline{0.924} & 0.965 \\
Claude-4.5-Opus         
& \textbf{0.923} & \textbf{0.965} & \underline{0.889} & 0.951 & \underline{0.909} & \textbf{0.974} & \textbf{0.899} & \textbf{0.955} & 0.884 & 0.952 & \textbf{0.931} & \underline{0.974} \\

\midrule
\multicolumn{13}{l}{\textbf{Open-Source in Retrieval-Augmented SQL Generation Methods}} \\
\cmidrule(lr){1-13}
Deepseek-R1-1.5B          
& 0.735 & 0.844 & 0.621 & 0.805 & 0.739 & 0.862 & 0.567 & 0.767 & 0.656 & 0.826 & 0.670 & 0.813 \\
Deepseek-R1-7B          
& 0.732 & 0.766 & 0.758 & 0.824 & 0.752 & 0.812 & 0.771 & 0.862 & 0.787 & 0.869 & 0.777 & 0.812 \\
Deepseek-R1-14B         
& 0.802 & 0.868 & 0.792 & 0.888 & 0.819 & 0.911 & 0.765 & 0.853 & 0.811 & 0.896 & 0.826 & 0.886 \\
Deepseek-R1-32B         
& 0.848 & 0.903 & 0.843 & 0.925 & 0.887 & 0.961 & 0.830 & 0.917 & 0.883 & 0.958 & 0.912 & \textbf{0.971} \\
Deepseek-V3.2-685B           
& \textbf{0.908} & \textbf{0.949} & \underline{0.873} & \textbf{0.949} & \textbf{0.908} & \underline{0.963} & \textbf{0.888} & \textbf{0.948} & \underline{0.898} & 0.958 & \textbf{0.924} & \textbf{0.971} \\
Qwen3-1.7B               
& 0.861 & 0.916 & 0.827 & 0.910 & 0.846 & 0.924 & 0.793 & 0.886 & 0.805 & 0.893 & 0.856 & 0.926 \\
Qwen3-8B               
& 0.903 & 0.936 & 0.862 & 0.940 & \underline{0.904} & 0.961 & 0.871 & 0.942 & 0.892 & 0.956 & 0.912 & 0.967 \\
Qwen3-14B                 
& 0.895 & 0.933 & 0.864 & 0.940 & 0.893 & \underline{0.963} & 0.869 & 0.938 & 0.897 & \textbf{0.963} & 0.910 & \underline{0.970} \\
Qwen3-32B        
& 0.896 & 0.935 & 0.859 & 0.937 & 0.902 & 0.962 & \underline{0.873} & 0.943 & \textbf{0.899} & \underline{0.962} & \underline{0.918} & \textbf{0.971} \\
Qwen3-235B-A22B       
& 0.894 & 0.942 & \textbf{0.877} & \underline{0.946} & 0.891 & \textbf{0.964} & 0.867 & \underline{0.947} & 0.893 & \underline{0.962} & 0.916 & \textbf{0.971} \\
%Llama-3.1-8B    
%& 0.640 & 0.807 & 0.696 & 0.852 & 0.724 & 0.867 & 0.778 & 0.892 & 0.869 & 0.950 & 0.874 & 0.943 \\
%Llama-3.1-70B    
%& -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%Llama-3.1-405B    
%& -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Gemma-2-2B          
& 0.879 & 0.931 & 0.820 & 0.907 & 0.842 & 0.921 & 0.841 & 0.919 & 0.824 & 0.901 & 0.851 & 0.924 \\
Gemma-2-9B          
& \underline{0.904} & \underline{0.944} & 0.865 & 0.942 & \underline{0.904} & 0.958 & 0.859 & 0.934 & 0.876 & 0.949 & 0.914 & 0.964 \\
\bottomrule
\end{tabular}

\caption{
Cosine similarity scores between predicted SQL results and gold SQL answers across the six benchmark task types:
single-table reasoning (level 0);
double-table key joins (level 1);
double-table spatial joins (level 2);
triple-table key--key joins (level 3);
triple-table key--spatial joins (level 4);
and triple-table spatial--spatial joins (level 5).
For each task type, we report scores computed with \textbf{OpenAI text-embedding-3-large} (OpenAI)
and \textbf{Jina Embeddings v3} (Jina).
All nine LLM--RAG agents are evaluated under the same RAG SQL generation framework as shown in Fig.~\ref{fig:rag}. The best results are \textbf{bold} while the second best results are \underline{underlined}.
}
\label{tab:benchmark-types}
\end{table*}


==> tables/llm_rag_comparisons_orignal_data.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{lcccccccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Level 0}} 
 & \multicolumn{2}{c}{\textbf{Level 1}} 
 & \multicolumn{2}{c}{\textbf{Level 2}} 
 & \multicolumn{2}{c}{\textbf{Level 3}} 
 & \multicolumn{2}{c}{\textbf{Level 4}} 
 & \multicolumn{2}{c}{\textbf{Level 5}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\textbf{Model} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} &
\textbf{OpenAI} & \textbf{Jina} \\
\midrule

\multicolumn{13}{l}{\textbf{Close-Source in Retrieval-Augmented SQL Generation Methods}} \\
\cmidrule(lr){1-13}
GPT-4o                  
& 0.914 & 0.962 & \textbf{0.891} & \textbf{0.957} & \underline{0.909} & \textbf{0.974} & 0.883 & \underline{0.951} & \textbf{0.904} & \textbf{0.962} & 0.919 & \textbf{0.976} \\
GPT-4.1                 
& 0.915 & 0.951 & 0.876 & 0.945 & 0.897 & 0.966 & 0.864 & 0.938 & 0.877 & 0.945 & 0.907 & 0.964 \\
GPT-5.1                 
& 0.917 & \underline{0.963} & 0.886 & \underline{0.953} & 0.899 & \underline{0.970} & 0.863 & 0.945 & 0.895 & 0.955 & 0.910 & 0.968 \\
Gemini-2.0-Flash-Lite$^*$   
& 0.897 & 0.934 & 0.869 & 0.945 & 0.907 & 0.962 & 0.885 & 0.948 & 0.874 & 0.943 & 0.914 & 0.964 \\
Gemini-2.5-Flash-Lite   
& 0.885 & 0.945 & 0.846 & 0.934 & 0.906 & 0.967 & 0.855 & 0.937 & 0.872 & 0.943 & 0.901 & 0.958 \\
Gemini-2.5-Pro          
& 0.887 & 0.943 & 0.872 & 0.952 & \textbf{0.914} & \textbf{0.974} & 0.862 & 0.940 & 0.883 & 0.955 & 0.923 & 0.970 \\
Claude-3-Haiku          
& \underline{0.919} & 0.957 & 0.862 & 0.939 & 0.895 & 0.960 & 0.870 & 0.947 & 0.895 & 0.957 & 0.895 & 0.960 \\
Claude-3.5-Haiku        
& 0.903 & 0.949 & 0.851 & 0.934 & 0.899 & 0.969 & 0.833 & 0.933 & \underline{0.898} & \underline{0.961} & 0.899 & 0.966 \\
Claude-4.5-Haiku$^*$        
& 0.900 & 0.952 & 0.870 & 0.938 & 0.896 & 0.966 & 0.879 & 0.949 & 0.895 & 0.958 & 0.921 & 0.973 \\
Claude-4.5-Sonnet         
& 0.907 & 0.950 & 0.856 & 0.931 & 0.904 & 0.969 & \underline{0.890} & \underline{0.951} & \textbf{0.904} & 0.952 & \underline{0.924} & 0.965 \\
Claude-4.5-Opus         
& \textbf{0.923} & \textbf{0.965} & \underline{0.889} & 0.951 & \underline{0.909} & \textbf{0.974} & \textbf{0.899} & \textbf{0.955} & 0.874 & 0.947 & \textbf{0.931} & \underline{0.974} \\

\midrule
\multicolumn{13}{l}{\textbf{Open-Source in Retrieval-Augmented SQL Generation Methods}} \\
\cmidrule(lr){1-13}
Deepseek-R1-1.5B$^*$          
& 0.735 & 0.844 & 0.621 & 0.805 & 0.739 & 0.862 & 0.567 & 0.767 & 0.585 & 0.786 & 0.670 & 0.813 \\
Deepseek-R1-7B$^*$         
& 0.732 & 0.766 & 0.758 & 0.824 & 0.752 & 0.812 & 0.771 & 0.862 & 0.776 & 0.843 & 0.777 & 0.812 \\
Deepseek-R1-14B$^*$          
& 0.802 & 0.868 & 0.792 & 0.888 & 0.819 & 0.911 & 0.765 & 0.853 & 0.803 & 0.882 & 0.826 & 0.886 \\
Deepseek-R1-32B$^*$          
& 0.848 & 0.903 & 0.843 & 0.925 & 0.887 & 0.961 & 0.830 & 0.917 & 0.889 & \underline{0.958} & 0.912 & \textbf{0.971} \\
Deepseek-V3.2-685B           
& \textbf{0.908} & \textbf{0.949} & \underline{0.873} & \textbf{0.949} & \textbf{0.908} & \underline{0.963} & \textbf{0.888} & \textbf{0.948} & \underline{0.896} & \underline{0.958} & \textbf{0.924} & \textbf{0.971} \\
Qwen3-1.7B               
& 0.861 & 0.916 & 0.827 & 0.910 & 0.846 & 0.924 & 0.793 & 0.886 & 0.824 & 0.900 & 0.856 & 0.926 \\
Qwen3-8B               
& 0.903 & 0.936 & 0.862 & 0.940 & \underline{0.904} & 0.961 & 0.871 & 0.942 & 0.875 & 0.946 & 0.912 & 0.967 \\
Qwen3-14B                 
& 0.895 & 0.933 & 0.864 & 0.940 & 0.893 & \underline{0.963} & 0.869 & 0.938 & 0.888 & 0.957 & 0.910 & \underline{0.970} \\
Qwen3-32B        
& 0.896 & 0.935 & 0.859 & 0.937 & 0.902 & 0.962 & \underline{0.873} & 0.943 & 0.893 & 0.957 & \underline{0.918} & \textbf{0.971} \\
Qwen3-235B-A22B       
& 0.894 & 0.942 & \textbf{0.877} & \underline{0.946} & 0.891 & \textbf{0.964} & 0.867 & \underline{0.947} & \textbf{0.898} & \textbf{0.962} & 0.916 & \textbf{0.971} \\
Gemma-2-2B$^*$          
& 0.879 & 0.931 & 0.820 & 0.907 & 0.842 & 0.921 & 0.841 & 0.919 & 0.818 & 0.909 & 0.851 & 0.924 \\
Gemma-2-9B          
& \underline{0.904} & \underline{0.944} & 0.865 & 0.942 & \underline{0.904} & 0.958 & 0.859 & 0.934 & 0.877 & 0.948 & 0.914 & 0.964 \\
\bottomrule
\end{tabular}

\caption{
Cosine similarity scores between predicted SQL results and gold SQL answers across the six benchmark task types:
single-table reasoning (level 0);
double-table key joins (level 1);
double-table spatial joins (level 2);
triple-table key--key joins (level 3);
triple-table key--spatial joins (level 4);
and triple-table spatial--spatial joins (level 5).
For each task type, we report scores computed with \textbf{OpenAI text-embedding-3-large} (OpenAI)
and \textbf{Jina Embeddings v3} (Jina).
All nine LLM--RAG agents are evaluated under the same RAG SQL generation framework as shown in Fig.~\ref{fig:rag}. The best results are \textbf{bold} while the second best results are \underline{underlined}. $^*$ indicates LLM agents that were unable to produce all valid SQL queries (failure cases exist), according to our best-effort examination.
}
\label{tab:benchmark-types}
\end{table*}

